Automatic Non-Linear Video Editing Transfer

We propose an automatic approach that extracts editing styles in a source video and applies the edits to matched footage for video creation. Our Computer Vision based techniques considers framing, content type, playback speed, and lighting of each input video segment. By applying a combination of these features, we demonstrate an effective method that automatically transfers the visual and temporal styles from professionally edited videos to unseen raw footage. We evaluated our approach with real-world videos that contained a total of 3872 video shots of a variety of editing styles, including different subjects, camera motions, and lighting. We reported feedback from survey participants who reviewed a set of our results.

==> 2_related_work.tex <==
% This section is wip and not included in the final paper

\section{Related Work}
Recent research has demonstrated advanced methods of high-quality style transfers. Gatys et al. Fine-grained attributes can be controlled, such as spatial and color information~\cite{NeuralStyleTransfer_2017} or semantic structure~\cite{AttributeTransfer_2017}. The performance can be stable in real-time~\cite{NeuralStyleTransferStability_2017} without pre-defined styles~\cite{10.5555/3294771.3294808}. Xia et al. proposed techniques that learn photorealistic attributes from one source image and applying to an unseen image~\cite{PhotorealisticStyleTransfer_2020}.

video per shot~\cite{StylizingVideobyExample_2019,10.1145/3386569.3392453,10.1145/3386569.3392457,CoherentOnlineVideoStyleTransfer_2017}

motion~\cite{RealtimeMotionStyleTransfer_2015}.

styles: quick cuts--style by text~\cite{DialogueDriven,transcript_2019,BScript_CHI2019}, viral videos~\cite{ViralVideoStyle_2014}

automatic video editing: fully automatic, with high-level markers~\cite{DemoCut_UIST13,QuickCut} or sources~\cite{URL2Video_UIST20} or heuristics~\cite{InterviewVideo}, metadata~\cite{MetadataVideoEditing_DIS02}

visualization~\cite{SchematicStoryboarding}


==> Automatic Non-Linear Editing (NLE) Style Transfer (2)/2_related_work.tex <==
% This section is wip and not included in the final paper

\section{Related Work}
Recent research has demonstrated advanced methods of high-quality style transfers. Gatys et al. Fine-grained attributes can be controlled, such as spatial and color information~\cite{NeuralStyleTransfer_2017} or semantic structure~\cite{AttributeTransfer_2017}. The performance can be stable in real-time~\cite{NeuralStyleTransferStability_2017} without pre-defined styles~\cite{10.5555/3294771.3294808}. Xia et al. proposed techniques that learn photorealistic attributes from one source image and applying to an unseen image~\cite{PhotorealisticStyleTransfer_2020}.

video per shot~\cite{StylizingVideobyExample_2019,10.1145/3386569.3392453,10.1145/3386569.3392457,CoherentOnlineVideoStyleTransfer_2017}

motion~\cite{RealtimeMotionStyleTransfer_2015}.

styles: quick cuts--style by text~\cite{DialogueDriven,transcript_2019,BScript_CHI2019}, viral videos~\cite{ViralVideoStyle_2014}

automatic video editing: fully automatic, with high-level markers~\cite{DemoCut_UIST13,QuickCut} or sources~\cite{URL2Video_UIST20} or heuristics~\cite{InterviewVideo}, metadata~\cite{MetadataVideoEditing_DIS02}

visualization~\cite{SchematicStoryboarding}


==> Automatic Non-Linear Editing (NLE) Style Transfer (2)/3_background.tex <==
\section{Background: Video Editing Techniques}
We build our work upon conventional video editing techniques that create effects on both visual and temporal domains of a video~\cite{arijon1991grammar,FilmArt_2013}. Video editors commonly combine multiple techniques to develop a unique editing style. Specifically, we focus on a subset of fundamental effects:
% We define some categories of modern effects and ways to represent them such that they can be transferred to new target footage.

\subheading{Framing} presents visual elements by considering the spatial placement of one or more subjects, which guide the audience's attention. Framing a series of video frames leads to the \emph{camera motion}, which is a core element of filmmaking.
A cinematic camera can move in multiple ways, including stationary and Pan–Tilt–Zoom (PTZ) that are commonly seen in user-generated videos. While unrestricted camera mounts allow for full six degrees of freedom (6DoF) motion, they are beyond our scope given the challenges of reproducing parallax effects on raw footage.
% 
% of a shot can be framed (positioned) at a location and distance depending on the goal of the clip.  Additionally, the camera's FOV may move during capture.

\subheading{Transition} is a mechanism to connect video shots temporally.
% Many transitions are defined by film makers based on the meaning they impart onto the content.  However, for this effort, directly transferring the transition from source to target footage allows for the skipping of classification.  
Common techniques include hard cuts (i.e., direct shot changes) and lighting-based transitions (e.g., fades) that we utilize in this work.  
% Shot transitions based on scene content and position are created through automatic adjacent scene framing.
% 
Transitions often consider the connection of content and framing between shots. Placements of subjects across multiple shots may create surprising effects, such as a ``match cut`` that intentionally aligns shapes, colors, and movements of two distinct shots~\cite{FilmArt_2013}.

\subheading{Playback speed} of a video segment adjusts the narrative pace, from slow (less than 1x), normal (1x), to fast (greater than 1x). Manipulating the speed often informs the importance or the emotion of a subject. For example, slow motion increases the drama of footage while high speed can increase the humor; speed ramps can enhance specific moments of a continuous action. %while reducing the duration of less interesting parts of the video.
% may be adjusted from is native real-time value (1x) to faster speeds (greater than 1x) or slower speeds (less than 1x).  In addition to fixed speeds, editors may adjust the speed dynamically in rigid patterns (e.g. speed ramp - piecewise linear) or even complex patterns where the playback speed is constantly changing.

% \subheading{Fading/Light Filtering/Lens Glare}
\subheading{Color and lighting} change the tone and mood of a video frame and can be adjusted during the capturing or the post-production phase. It is common that scenes in an edited video have applied color filters and lighting adjustments to enhance storytelling. 
% For example, scaling of brightness can help match a background music track or drive a new meaning. 
% Adjusting of brightness is also a popular editing technique to change the style or mood of a video.  
% Regardless of how they were originally applied, many color and lighting effects can measured and reproduced on new footage using only post-production editing.

==> Automatic Non-Linear Editing (NLE) Style Transfer (2)/6_results_discussion.tex <==
\newcommand{\numberOfProcessedVideos}[1] {60}
\newcommand{\numberOfProcessedVideoShots}[1] {3,872}
\newcommand{\numberOfSurveyResponses}[1] {15}
\newcommand{\numberOfSurveyResponsesToVideos}[1] {105}
\newcommand{\userquote}[1]{``\emph{#1}''}


\begin{figure}[t!]
\centerline{\includegraphics[trim=140 60 150 60,clip,width=0.88\columnwidth]{fig/review_UI.png}}
\caption{We visualize editing results in a review panel that include (A) the original source video annotated by keypoints, (B) the mosaic form of the captured camera motion, (C-D) the synchronized video timelines of the source and target videos showing shot changes, (E) subcropping of target footage that matches the camera motion of the mosaic, and (F) the output video.}
\label{fig:review}
\end{figure}

\section{Experiments}

% The accompanying demo videos show the original source footage used for edit style, the output video edited to the style of the source as well as debugging information.

We selected \numberOfProcessedVideos{} professional-edited videos from multiple creators on YouTube as the source videos to test our pipeline. We built our test set based on the following criteria: a video (1) includes more than 10 shots showing different subjects, (2) contains a mixture of camera views, and (3) has independent sound track.
%
The source videos are 2-minute long on average.
% 
The repository of target footage contains 40 raw videos, ranging from 30 to 90 seconds long.

\subsection{Results}

% and selected 7 partial videos used in an online survey. Below we report our observations and audience feedback.
Table~\ref{tab:result_analysis} presents the analysis of our results on \numberOfProcessedVideos{} videos. Figure~\ref{fig:reuslts} shows our example videos.
We reviewed the results using a visualization UI (see Figure~\ref{fig:review}).
Our pipeline detected a total of \numberOfProcessedVideoShots{} shots that include both long and short video shots of various content types and visual tones.
% 
We observed that the pipeline especially well captured camera motions, which can be difficult for average creators to edit and transfer manually without assistance. In addition, the pipeline selected and positioned subjects from raw footage similar to source videos with the exact temporal allocation. The combination of these editing decisions therefore provides a similar style.

% We present a demo reel of examples produced by the system here:
% \url{https://youtu.be/pd4qMP7y-cY}
% or here:
% \url{https://drive.google.com/file/d/1zgvj-ew4fvPRKyOq_SvOfWfgh2b4PJLs/view?usp=sharing}

\subsection{Audience Feedback}

To gather audience feedback, we conducted an online survey within our organization. Each survey participant was asked to review 7 selected video segments, each was 10 to 20 seconds long and contained 3-6 shots. We synchronized the source and output videos, presented side-by-side as one video for review. Each video was followed by three Likert-scale questions on the matches of \emph{editing style}, \emph{camera motion}, and \emph{visual quality} between the source and output videos. We also collected text comments.

We received \numberOfSurveyResponses{} responses with a total of \numberOfSurveyResponsesToVideos{} ratings to the videos per question. Overall, participants agreed that the editing style between the source and output videos is similar ($Median=4$ overall and for six of the seven videos), as well as the camera motion ($M=4$ overall and for all videos). They commented, \userquote{it's (the result video is) almost as good as the left one (the source video).} (on Test Video \# 4) and \userquote{very consistent motion} (on Test Video \# 2).
% 
We also learned that when comparing styles, people paid attention to the subjects, resolution, and quality carefully, while we received a neutral rating to the similarity of visual quality ($M=3$). One participant commented, \userquote{right video has some visible artifacts like video slowdown which was obviously filmed in lower fps — this completely breaks the immersion.} (on Test Video \# 3), and another noted, \userquote{resolution and camera focus on right video is inconsistent.} (on Test Video \# 5).
% 
These findings inspire us to focus effort on quality understanding, super resolution, and storytelling that we are currently developing.

% limitation, future opportunities, etc.

\begin{table}[t!]
\caption{We performed style extraction on 60 online videos, resulting in \numberOfProcessedVideoShots{} shots with a variety of content and motions.}
\centerline{\includegraphics[trim=200 80 200 60,clip,width=.99\columnwidth]{fig/analysis.pdf}} %left bottom right top
\label{tab:result_analysis}
\end{table}

\begin{figure}[t!]
\centerline{\includegraphics[trim=100 50 180 30,clip,width=0.95\columnwidth]{fig/results.png}}
\caption{Example results from our pipeline.}
\label{fig:reuslts}
\end{figure}
